Local Second-Order Limit Dynamics of the Alternating Direction Method of Multipliers for Semidefinite Programming

The alternating direction method of multipliers (ADMM) is widely used for solving large-scale semidefinite programs (SDPs), yet on instances with multiple primal-dual optimal solution pairs, it often enters prolonged slow-convergence regions where the Karush-Kuhn-Tucker (KKT) residuals nearly stall. To explain and predict the fine-grained dynamical behavior inside these regions, we develop a local second-order limit dynamics framework for ADMM near an arbitrary KKT point -- not necessarily the eventual limit point of the iterates. Assuming the existence of a strictly complementary primal-dual solution pair, we derive a second-order local expansion of the ADMM dynamics by leveraging a refined and simplified variational characterization of the (parabolic) second-order directional derivative of the PSD projection operator. This expansion reveals a closed convex cone of directions along which the local first-order update vanishes, and it induces a second-order limit map that governs the persistent drift after transient effects are filtered out. We characterize fundamental properties of this mapping, including its kernel, range, and continuity. A primal-dual decoupling further yields a clean scaling law for the effect of the penalty parameter in ADMM. We connect these properties to second-order dynamical features of ADMM, including fixed points, almost-invariant sets, and microscopic phases. Three empirical phenomena in slow-convergence regions are then explained or predicted: (i) angles between consecutive iterate differences are small yet nonzero, except for sparse spikes; (ii) primal and dual infeasibilities are insensitive to penalty-parameter updates; and (iii) iterates can be transiently trapped in a low-dimensional subspace for an extended period. Extensive numerical experiments on the Mittelmann dataset corroborate our theoretical predictions.

==> figs/field1/fig.tex <==
%!TEX root = ../main.tex

\begin{figure}[htbp]
    \centering

    \begin{minipage}{\textwidth}
        \centering
        \begin{tabular}{cc}
            \begin{minipage}{0.45\textwidth}
                \centering
                \includegraphics[width=\columnwidth]{figs/field1/Z_diff_norm.png}
            \end{minipage}

            \begin{minipage}{0.45\textwidth}
                \centering
                \includegraphics[width=\columnwidth]{figs/field1/Z_diff_ang.png}
            \end{minipage}
        \end{tabular}
    \end{minipage}
    \caption{Example~\ref{ex:soadmm:field1}: Experiment I. $a = 1, b = 1$, $t = 10^{-2}, 10^{-3}, 10^{-4}, 10^{-5}$, respectively. \label{fig:soadmm:field1}}
\end{figure}

==> figs/linesearch/fig_linesearch_comp.tex <==
%!TEX root = ../main.tex

\begingroup

\newcommand{\FieldFig}[2]{
    % first arg: dataset name; second arg: textwidth
    \begin{minipage}{#2\textwidth}
        \centering
        \dataset{#1}
        \includegraphics[width=\columnwidth]{\accPrefix/#1/linesearch_kkt_comp_data.png}
    \end{minipage}
}

\begin{figure}[htbp]
    \centering
    \begin{minipage}{\textwidth}
        \centering
        \includegraphics[width=0.5\columnwidth]{\accPrefix/1dc1024/linesearch_kkt_comp_legend.png}
        \vspace{3mm}
    \end{minipage}

    \begin{minipage}{\textwidth}
        \centering
        \begin{tabular}{ccccc}
            \FieldFig{1dc1024}{0.18}
            \FieldFig{1tc2048}{0.18}
            \FieldFig{cancer100}{0.18}
            \FieldFig{cnhil10}{0.18}
            \FieldFig{foot}{0.18}
        \end{tabular}
    \end{minipage}

    \begin{minipage}{\textwidth}
        \centering
        \begin{tabular}{ccccc}
            \FieldFig{G40mb}{0.18}
            \FieldFig{hand}{0.18}
            \FieldFig{neosfbr25}{0.18}
            \FieldFig{neosfbr30e8}{0.18}
            \FieldFig{neu1g}{0.18}
        \end{tabular}
    \end{minipage}

    \begin{minipage}{\textwidth}
        \centering
        \begin{tabular}{ccccc}
            \FieldFig{neu2g}{0.18}
            \FieldFig{neu3g}{0.18}
            \FieldFig{r12000}{0.18}
            \FieldFig{swissroll}{0.18}
            \FieldFig{texture}{0.18}
        \end{tabular}
    \end{minipage}

    \caption{\label{fig:exp:linesearch-kkt-comp} $r_{\max}$ comparison between Baseline and Line-Search for $15$ hard-to-solve \Mittelmann~SDP datasets (single-block, block size $\le 3000$).}
\end{figure}

\endgroup

==> figs/original/fig_baseline_obj.tex <==
%!TEX root = ../main.tex

\begingroup

\newcommand{\FieldFig}[2]{
    % first arg: dataset name; second arg: textwidth
    \begin{minipage}{#2\textwidth}
        \centering
        \dataset{#1}
        \includegraphics[width=\columnwidth]{\accPrefix/#1/baseline_obj_data.png}
    \end{minipage}
}

\begin{figure}[htbp]
    \centering
    \begin{minipage}{\textwidth}
        \centering
        \includegraphics[width=0.5\columnwidth]{\accPrefix/1dc1024/baseline_obj_legend.png}
        \vspace{3mm}
    \end{minipage}

    \begin{minipage}{\textwidth}
        \centering
        \begin{tabular}{ccccc}
            \FieldFig{1dc1024}{0.18}
            \FieldFig{1tc2048}{0.18}
            \FieldFig{cancer100}{0.18}
            \FieldFig{cnhil10}{0.18}
            \FieldFig{foot}{0.18}
        \end{tabular}
    \end{minipage}

    \begin{minipage}{\textwidth}
        \centering
        \begin{tabular}{ccccc}
            \FieldFig{G40mb}{0.18}
            \FieldFig{hand}{0.18}
            \FieldFig{neosfbr25}{0.18}
            \FieldFig{neosfbr30e8}{0.18}
            \FieldFig{neu1g}{0.18}
        \end{tabular}
    \end{minipage}

    \begin{minipage}{\textwidth}
        \centering
        \begin{tabular}{ccccc}
            \FieldFig{neu2g}{0.18}
            \FieldFig{neu3g}{0.18}
            \FieldFig{r12000}{0.18}
            \FieldFig{swissroll}{0.18}
            \FieldFig{texture}{0.18}
        \end{tabular}
    \end{minipage}

    \caption{\label{fig:exp:baseline-obj} AAA.}
\end{figure}

\endgroup

==> figs/original/fig_original_comp.tex <==
%!TEX root = ../main.tex

\begingroup

\newcommand{\FieldFig}[2]{
    % first arg: dataset name; second arg: textwidth
    \begin{minipage}{#2\textwidth}
        \centering
        \dataset{#1}
        \includegraphics[width=\columnwidth]{\accPrefix/#1/original_data.png}
    \end{minipage}
}

\begin{figure}[htbp]
    \centering
    \begin{minipage}{\textwidth}
        \centering
        \includegraphics[width=0.5\columnwidth]{\accPrefix/1dc1024/original_legend.png}
        \vspace{3mm}
    \end{minipage}

    \begin{minipage}{\textwidth}
        \centering
        \begin{tabular}{ccccc}
            \FieldFig{1dc1024}{0.18}
            \FieldFig{1et2048}{0.18}
            \FieldFig{1tc2048}{0.18}
            \FieldFig{1zc1024}{0.18}
            \FieldFig{cancer100}{0.18}
        \end{tabular}
    \end{minipage}

    \begin{minipage}{\textwidth}
        \centering
        \begin{tabular}{ccccc}
            \FieldFig{cnhil10}{0.18}
            \FieldFig{cphil12}{0.18}
            \FieldFig{foot}{0.18}
            \FieldFig{G40mb}{0.18}
            \FieldFig{G48mb}{0.18}
        \end{tabular}
    \end{minipage}

    \begin{minipage}{\textwidth}
        \centering
        \begin{tabular}{ccccc}
            \FieldFig{G48mc}{0.18}
            \FieldFig{hamming8}{0.18}
            \FieldFig{hamming9}{0.18}
            \FieldFig{hand}{0.18}
            \FieldFig{neosfbr25}{0.18}
        \end{tabular}
    \end{minipage}

    \begin{minipage}{\textwidth}
        \centering
        \begin{tabular}{ccccc}
            \FieldFig{neosfbr30e8}{0.18}
            \FieldFig{neu1g}{0.18}
            \FieldFig{neu2g}{0.18}
            \FieldFig{neu3g}{0.18}
            \FieldFig{r12000}{0.18}
        \end{tabular}
    \end{minipage}

    \begin{minipage}{\textwidth}
        \centering
        \begin{tabular}{ccccc}
            \FieldFig{swissroll}{0.18}
            \FieldFig{theta12}{0.18}
            \FieldFig{theta102}{0.18}
            \FieldFig{theta123}{0.18}
            \FieldFig{texture}{0.18}
        \end{tabular}
    \end{minipage}

    \caption{\label{fig:exp:original} $r_{\max}$, $\normF{\Delta \Vark{Z}}$, and $\angle (\Delta \Vark{Z}, \Delta \Varkpo{Z})$ for $25$ \Mittelmann~SDP datasets (single-block, block size $\le 3000$). For \emph{all} SDP instances exhibiting slow convergence, $\angle (\Delta \Vark{Z}, \Delta \Varkpo{Z})$ remains small for a long time. In comparison, for many SDP instances achieving observable sharp linear convergence, $\angle (\Delta \Vark{Z}, \Delta \Varkpo{Z})$ is large.}
\end{figure}

\endgroup

==> figs/sigwave/fig_sigwave_comp.tex <==
%!TEX root = ../main.tex

\begingroup

\newcommand{\FieldFig}[2]{
    % first arg: dataset name; second arg: textwidth
    \begin{minipage}{#2\textwidth}
        \centering
        \dataset{#1}
        \includegraphics[width=\columnwidth]{\accPrefix/#1/sigwave_kkt_comp_data.png}
    \end{minipage}
}

\begin{figure}[htbp]
    \centering
    \begin{minipage}{\textwidth}
        \centering
        \includegraphics[width=0.5\columnwidth]{\accPrefix/1dc1024/sigwave_kkt_comp_legend.png}
        \vspace{3mm}
    \end{minipage}

    \begin{minipage}{\textwidth}
        \centering
        \begin{tabular}{ccccc}
            \FieldFig{1dc1024}{0.18}
            \FieldFig{1tc2048}{0.18}
            \FieldFig{cancer100}{0.18}
            \FieldFig{cnhil10}{0.18}
            \FieldFig{foot}{0.18}
        \end{tabular}
    \end{minipage}

    \begin{minipage}{\textwidth}
        \centering
        \begin{tabular}{ccccc}
            \FieldFig{G40mb}{0.18}
            \FieldFig{hand}{0.18}
            \FieldFig{neosfbr25}{0.18}
            \FieldFig{neosfbr30e8}{0.18}
            \FieldFig{neu1g}{0.18}
        \end{tabular}
    \end{minipage}

    \begin{minipage}{\textwidth}
        \centering
        \begin{tabular}{ccccc}
            \FieldFig{neu2g}{0.18}
            \FieldFig{neu3g}{0.18}
            \FieldFig{r12000}{0.18}
            \FieldFig{swissroll}{0.18}
            \FieldFig{texture}{0.18}
        \end{tabular}
    \end{minipage}

    \caption{\label{fig:exp:sigwave-kkt-comp} $r_{\max}$ comparison between Baseline and Penalty-Wave for $15$ hard-to-solve \Mittelmann~SDP datasets (single-block, block size $\le 3000$).}
\end{figure}

\endgroup

==> figs/sigwave/fig_sigwave_study_Ampl=10.tex <==
%!TEX root = ../main.tex

\begingroup

\newcommand{\FieldFig}[2]{
    % first arg: dataset name; second arg: textwidth
    \begin{minipage}{#2\textwidth}
        \centering
        \dataset{#1}
        \includegraphics[width=\columnwidth]{\sigPrefix/#1/diff_norm_Ampl=10_N=20000.png}
        \includegraphics[width=\columnwidth]{\sigPrefix/#1/anchor_ang_Ampl=10_N=20000.png}
    \end{minipage}
}

\begin{figure}[htbp]
    \centering
    \begin{minipage}{\textwidth}
        \centering
        \includegraphics[width=0.5\columnwidth]{\sigPrefix/1dc1024/legend.png}
        \vspace{3mm}
    \end{minipage}

    \begin{minipage}{\textwidth}
        \centering
        \begin{tabular}{ccccc}
            \FieldFig{1dc1024}{0.18}
            \FieldFig{1tc2048}{0.18}
            \FieldFig{cancer100}{0.18}
            \FieldFig{cnhil10}{0.18}
            \FieldFig{foot}{0.18}
        \end{tabular}
    \end{minipage}

    \begin{minipage}{\textwidth}
        \centering
        \begin{tabular}{ccccc}
            \FieldFig{G40mb}{0.18}
            \FieldFig{hand}{0.18}
            \FieldFig{neosfbr25}{0.18}
            \FieldFig{neosfbr30e8}{0.18}
            \FieldFig{neu1g}{0.18}
        \end{tabular}
    \end{minipage}

    \begin{minipage}{\textwidth}
        \centering
        \begin{tabular}{ccccc}
            \FieldFig{neu2g}{0.18}
            \FieldFig{neu3g}{0.18}
            \FieldFig{r12000}{0.18}
            \FieldFig{swissroll}{0.18}
            \FieldFig{texture}{0.18}
        \end{tabular}
    \end{minipage}

    \caption{\label{fig:exp:sigwave-Ampl=10} AAA.}
\end{figure}

\endgroup

==> figs/toy1/fig_taskI.tex <==
%!TEX root = ../main.tex

\begin{figure}[htbp]
    \centering

    \begin{minipage}{\textwidth}
        \centering
        \begin{tabular}{cccc}
            \begin{minipage}{0.24\textwidth}
                \centering
                \includegraphics[width=\columnwidth]{\toyPrefix/toy1/taskI_Znorm_comp.png}
                (a)
            \end{minipage}

            \begin{minipage}{0.24\textwidth}
                \centering
                \includegraphics[width=\columnwidth]{\toyPrefix/toy1/taskI_Zang_comp.png}
                (b)
            \end{minipage}

            \begin{minipage}{0.24\textwidth}
                \centering
                \includegraphics[width=\columnwidth]{\toyPrefix/toy1/taskI_mdvZ_relerr_comp.png}
                (c)
            \end{minipage}

            \begin{minipage}{0.24\textwidth}
                \centering
                \includegraphics[width=\columnwidth]{\toyPrefix/toy1/taskI_mdvZ_instant_relerr_comp.png}
                (d)
            \end{minipage}
        \end{tabular}
    \end{minipage}
    \caption{\label{fig:toy1:taskI} AAA}
\end{figure}

==> figs/toy1/fig_taskIV.tex <==
%!TEX root = ../main.tex

\begin{figure}[htbp]
    \centering

    \begin{minipage}{\textwidth}
        \centering
        \includegraphics[width=0.4\columnwidth]{\toyPrefix/toy1/taskIV_legend.png}
        % \vspace{3mm}
    \end{minipage}

    \begin{minipage}{\textwidth}
        \centering
        \begin{tabular}{cccc}
            \begin{minipage}{0.24\textwidth}
                \centering
                \includegraphics[width=\columnwidth]{\toyPrefix/toy1/taskIV_tinv=100.png}
                (a) $t = 10^{-2}$
            \end{minipage}

            \begin{minipage}{0.24\textwidth}
                \centering
                \includegraphics[width=\columnwidth]{\toyPrefix/toy1/taskIV_tinv=1000.png}
                (b) $t = 10^{-3}$
            \end{minipage}

            \begin{minipage}{0.24\textwidth}
                \centering
                \includegraphics[width=\columnwidth]{\toyPrefix/toy1/taskIV_tinv=10000.png}
                (c) $t = 10^{-4}$
            \end{minipage}

            \begin{minipage}{0.24\textwidth}
                \centering
                \includegraphics[width=\columnwidth]{\toyPrefix/toy1/taskIV_tinv=100000.png}
                (d) $t = 10^{-5}$
            \end{minipage}
        \end{tabular}
    \end{minipage}

    \caption{\label{fig:toy:toy1-taskIV} Fixing $\ZHbar$. In each $t$, run $2000$ ADMM iterations, with $\log_{10}(\sigma)$ growing uniformly from $0$ to $1$. In the numerical results, as $t \downarrow 0$, $\log_{10}(\Delta \Vark{X})$ and $\log_{10}(\Delta \Vark{S})$ are linear in $\log_{10}(\sigma)$, while $\log_{10}(\Vark{r}_p)$ and $\log_{10}(\Vark{r}_d)$ are almost two constant lines.}
\end{figure}

==> figs/toy1/fig_taskV.tex <==
%!TEX root = ../main.tex

\begin{figure}[htbp]
    \centering

    \begin{minipage}{\textwidth}
        \centering
        \begin{tabular}{cc}
            \begin{minipage}{0.45\textwidth}
                \centering
                \includegraphics[width=\columnwidth]{\toyPrefix/toy1/taskV_tinv=100.png}
                (a) $t = 10^{-2}$
            \end{minipage}

            \begin{minipage}{0.45\textwidth}
                \centering
                \includegraphics[width=\columnwidth]{\toyPrefix/toy1/taskV_tinv=1000.png}
                (b) $t = 10^{-3}$
            \end{minipage}
        \end{tabular}
    \end{minipage}

    \begin{minipage}{\textwidth}
        \centering
        \begin{tabular}{cc}
            \begin{minipage}{0.45\textwidth}
                \centering
                \includegraphics[width=\columnwidth]{\toyPrefix/toy1/taskV_tinv=10000.png}
                (a) $t = 10^{-4}$
            \end{minipage}

            \begin{minipage}{0.45\textwidth}
                \centering
                \includegraphics[width=\columnwidth]{\toyPrefix/toy1/taskV_tinv=100000.png}
                (b) $t = 10^{-5}$
            \end{minipage}
        \end{tabular}
    \end{minipage}

    \caption{\label{fig:toy:toy1-taskV} $\Vark{Z}$'s trajectories from different $Z^{(0)}$ initialization with different $t$'s and first-order perturbation matrix $H$'s. $t$ is swept from $10^{-2}$ to $10^{-4}$. For each fixed $t$, $(H_{11}, H_{12}, H_{22})$ is sampled from $\{-2, -1, 1, -2\}^3$, $64$ points in total. Observations: (1) from all initial points, it only takes one ADMM iteration for $\Vark{Z}$'s to collapse to $\ker(\deltafirst)$, regardless of $t$'s choices. (2) As $t \downarrow 0$, $\Vark{Z}$'s update in $\ker(\deltafirst)$ becomes slower, with each iteration's growth converging to the second-order limiting dynamics.}
\end{figure}
